MMGR: Multi-Modal Generative Reasoning Benchmark and Evaluation

Modern multimodal generative models can synthesize visually compelling images and videos, but it remains unclear whether this visual fluency reflects genuine reasoning: when prompted to generate a solution, can a model preserve the physical, logical, spatial, and temporal constraints a task requires, or does it merely produce plausible-looking media? To answer this question, we introduce MMGR (Multi-Modal Generative Reasoning Benchmark and Evaluation), a benchmark for evaluating generative reasoning across video, image, and language-based systems. MMGR covers 10 tasks from three domains (Abstract Reasoning, Embodied Navigation, and Physical Commonsense) and probes five reasoning abilities: Physical, Logical, 2D Spatial, 3D Spatial, and Temporal. Its evaluation emphasizes answer-verifiable tasks and, for video generation, process-aware chain-of-frame reasoning, where intermediate frames must form valid steps toward the target outcome rather than visually smooth but incorrect transitions. Evaluating state-of-the-art video generators, image generators, and LLM/VLM baselines reveals a sharp gap between visual quality and reasoning correctness: video models perform best on Physical Commonsense, but remain weak on symbolic tasks such as Sudoku, ARC, and Math, and brittle in cross-view embodied navigation. Image generators often outperform video generators on embodied navigation despite lacking temporal outputs, showing that longer visual generation does not automatically yield stronger reasoning. MMGR reframes evaluation of multimodal generation from whether outputs look realistic to whether they solve the underlying reasoning problem.

==> tables/arc_agreement_results.tex <==
\begin{table}[t]
\centering
\small
% \vspace{-2mm}
\caption{Human–VLM evaluator agreement on the \textbf{ARC} and \textbf{Physics} tasks (Veo-3). We report accuracy (\%) and Cohen's $\kappa$.}

\noindent
\begin{minipage}[t]{0.46\linewidth}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{@{}l|cc@{}}
    \toprule
    \textbf{Metric} & Acc. & $\kappa$ \\
    \midrule
    Pattern Recognition & 78.57 & 0.273 \\
    Grid Integrity      & 67.35 & 0.220 \\
    Color Accuracy      & 74.49 & 0.093 \\
    \midrule
    \textbf{Overall Score} & 94.90 & 0.000 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \subcaption{ARC (n=98 samples)}
\end{minipage}%  <-- THIS % IS CRITICAL
\hfill
\begin{minipage}[t]{0.46\linewidth}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{@{}l|cc@{}}
    \toprule
    \textbf{Metric} & Acc. & $\kappa$ \\
    \midrule
    Physics Accuracy & 67.3 & 0.231 \\
    Prompt Adherence & 71.4 & 0.284 \\
    Visual Realism   & 91.8 & 0.000 \\
    Motion Quality   & 91.8 & 0.000 \\
    \midrule
    \textbf{Overall Score} & 91.8 & 0.000 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \subcaption{Physics (n=49 samples)}
    \vspace{-5mm}
\end{minipage}
\vspace{-4mm}
\label{tab:agreement_results}
\end{table}

==> tables/embodied_agreement_results.tex <==
\begin{table*}[h!]
\centering
\scriptsize
\caption{Human-VLM evaluator agreement across four \textbf{embodied navigation} tasks (Veo-3). Metrics are grouped into Success and Consistency categories. We report raw agreement accuracy (\%) and Cohen's $\kappa$ for each evaluation metric.}
\label{tab:embodied_agreement_combined}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}ll|cc|cc|cc@{}}
\toprule
& & \multicolumn{2}{c|}{\textbf{Last-Mile Nav.}} & \multicolumn{2}{c|}{\textbf{Top-down View Nav.}} & \multicolumn{2}{c}{\textbf{3D R.-W. Nav.}}  \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
\textbf{Category} & \textbf{Metric} & Acc & $\kappa$ & Acc & $\kappa$ & Acc & $\kappa$ \\
\midrule
\multirow{4}{*}{VLM-based}
% & Success Score     & 80.00 (3D) & 0.514 & 66.67 (2D) & 0.342 & 80.00 (3D) & 0.552 & 38.46 (2D) / 53.85 (3D) & -0.268 / 0.025 \\
& Success Score 2D  & -- & -- & 50.00 & 0.043  & -- & --\\
& Success Score 3D  & 66.67 & 0.3478  & -- & -- & 76.67 & 0.462\\
% \midrule
% & Oracle Success Score  & 80.00 (3D) & 0.480 & 70.00 (2D) & 0.000 & 76.67 (3D) & 0.386 & 30.77 (2D) / 30.77 (3D) & -0.345 / -0.377 \\
& Oracle Success Score 2D & -- & -- & 33.33 & -0.333  & -- & -- \\
& Oracle Success Score 3D  & 53.33 &  0.1772  & -- & -- & 73.33 & 0.2638\\
\midrule

\multirow{2}{*}{Geo-Align / View-Syn}
& SR vs S.S. 2D  & -- & -- & &\\
& SR vs S.S. 3D & 51.72 & 13.62 & -- & --\\
& SR vs O.S. 2D & -- & -- & & \\
& SR vs O.S. 3D & 55.17 & 17.86\\


% \midrule
% & Trajectory Alignment Score & -- & -- & -- & -- & -- & -- & 53.85 & 0.000 \\
% \midrule
% \multirow{6}{*}{Consistency}
% & Object Semantic Score       & 84.44 & 0.154 & 53.33 & 0.129 & 76.67 & 0.000 & 46.15 & 0.042 \\
% & Agent Consistency Score     & 84.44 & -0.083 & 43.33 & 0.038 & 76.67 & 0.000 & 38.46 & -0.209 \\
% & Spatial Alignment Score     & 91.11 & -0.044 & 46.67 & 0.121 & 36.67 & 0.000 & 46.15 & -0.124 \\
% & Destination Integrity Score & 62.22 & 0.207 & 50.00 & 0.059 & 56.67 & 0.177 & 38.46 & -0.020 \\
% & Scene Consistency Score     & 68.89 & 0.035 & 30.00 & 0.025 & 56.67 & 0.133 & 38.46 & -0.156 \\
% \midrule
% & \textbf{Overall Score} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/maze_agreement_results.tex <==
\begin{table}[t]
\centering
\small
\caption{Human–evaluator agreement on the \textbf{Maze} task across three video models (n=540 total samples). We report raw agreement accuracy (\%) and Cohen's $\kappa$ for each evaluation metric.}
\vspace{-2mm}

\begin{subtable}{\columnwidth}
\centering
\caption*{(Top) Human vs. Pixel-based Evaluator}
\vspace{-2mm}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
\textbf{Metrics} & \multicolumn{2}{c|}{\textbf{CW}} & \multicolumn{2}{c|}{\textbf{MC}} &
  \multicolumn{2}{c|}{\textbf{AR}} & \multicolumn{2}{c|}{\textbf{TA}} &
  \multicolumn{2}{c}{\textbf{OS}} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & Acc. & $\kappa$ & Acc. & $\kappa$ & Acc. & $\kappa$
& Acc. & $\kappa$ & Acc. & $\kappa$ \\
\midrule
% Sora-2 & 78.3 & 0.026 &  &  & 56.7 & 0.117 & 71.7 & 0.342 & 98.3 & 0.000 \\
Veo-3 & 85.82 & 0.163 & 35.82 & 0.031 & 57.46 & 0.139 & 28.36 & -0.015 & 0.910 & 0.099 \\
% Wan-2.2 & 93.3 & 0.000 &  &  & 58.3 & 0.102 & 65.0 & 0.287 & 100.0 & 1.000 \\
% \midrule
% \textbf{Avg.} & 82.8 & 0.205 &  &  & 56.7 & 0.138 & 68.3 & 0.348 & 99.4 & 0.667 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{subtable}

\vspace{1mm}

\begin{subtable}{\columnwidth}
\centering
\caption*{(Bottom) Human vs. VLM-based Evaluator}
\vspace{-2mm}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
& \multicolumn{2}{c|}{\textbf{CW}} & \multicolumn{2}{c|}{\textbf{MC}} &
  \multicolumn{2}{c|}{\textbf{AR}} & \multicolumn{2}{c|}{\textbf{TA}} &
  \multicolumn{2}{c}{\textbf{OS}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & Acc. & $\kappa$ & Acc. & $\kappa$ & Acc. & $\kappa$
& Acc. & $\kappa$ & Acc. & $\kappa$ \\
\midrule
% Sora-2  &  &  &  &  &  &  &  &  &  &  \\
Veo-3 & 35.00 & 0.085 & 72.50 & -0.048 & 40.00 & 0.000 & 65.00 & 0.300 & 45.00 & -0.055 \\
% Wan-2.2 &  &  &  &  &  &  &  &  &  &  \\
% \midrule
% \textbf{Avg.} &  &  &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{subtable}
\vspace{-5mm}
\label{tab:maze_agreement_combined}
\end{table}

==> tables/maze_human_results.tex <==
\begin{table*}[h!]
\centering
\small
\caption{Comparison of \textbf{Auto-Eval} (VLM-based) and \textbf{Human-Eval} results for \textbf{Veo-3} on the 2D Maze task across two maze generation algorithms (DFS and Wilson's) and three difficulty levels (Easy, Medium, and Hard).}
\label{tab:maze_human_results}
\begin{adjustbox}{max width=\textwidth}
{
\begin{tabular}{@{}l|ccccc|ccccc@{}}
\toprule
& \multicolumn{5}{c|}{\textbf{Auto-Eval}} & \multicolumn{5}{c}{\textbf{Human-Eval}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}

\textbf{Setting}
& \textbf{MC} $\downarrow$
& \textbf{CW} $\downarrow$
& \textbf{AR} $\uparrow$
& \textbf{TA} $\uparrow$
& \textbf{Overall} $\uparrow$
& \textbf{MC} $\downarrow$
& \textbf{CW} $\downarrow$
& \textbf{AR} $\uparrow$
& \textbf{TA} $\uparrow$
& \textbf{Overall} $\uparrow$ \\
\midrule

\multicolumn{11}{@{}l}{\textbf{Generator: Depth-First Search}} \\

\quad Easy (3$\times$3–5$\times$5)
& 15.50\% & 25.50\% & 1.00\% & 60.50\% & 42.00\%
& 36.67\% & 76.67\% & 60.00\% & 80.00\% & 10.00\% \\

\quad Medium (6$\times$6–9$\times$9)
& 0.50\% & 25.63\% & 0.00\% & 50.75\% & 38.69\%
& 23.33\% & 100.00\% & 13.33\% & 86.67\% & 0.00\% \\

\quad Hard (10$\times$10–13$\times$13)
& 0.00\% & 18.50\% & 1.50\% & 60.00\% & 51.50\%
& 20.00\% & 100.00\% & 26.67\% & 73.33\% & 0.00\% \\

\midrule
\multicolumn{11}{@{}l}{\textbf{Generator: Wilson's Algorithm}} \\

\quad Easy (3$\times$3–5$\times$5)
& 3.50\% & 21.50\% & 2.50\% & 61.50\% & 46.50\%
& 30.00\% & 76.67\% & 36.67\% & 90.00\% & 23.33\% \\

\quad Medium (6$\times$6–9$\times$9)
& 1.25\% & 15.63\% & 1.25\% & 55.63\% & 47.50\%
& 53.33\% & 96.67\% & 23.33\% & 76.67\% & 3.33\% \\

\quad Hard (10$\times$10–13$\times$13)
& 1.25\% & 18.75\% & 0.63\% & 58.75\% & 45.63\%
& 23.33\% & 100.00\% & 26.67\% & 83.33\% & 0.00\% \\

\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{0.5em}
\footnotesize
\textit{Note: MC = Maze Changed, CW = Cross Wall, AR = Action Reflection, TA = Target Achievement.}
\end{table*}

==> tables/physics_agreement_results.tex <==
\begin{table}[h!]
\centering
\small
\caption{Human-VLM evaluator agreement on the \textbf{Physics} task for Veo-3 ($n=49$ samples). We report accuracy (\%) and Cohen's $\kappa$.}
\label{tab:physics_agreement}
\begin{adjustbox}{max width=0.5\textwidth}
\begin{tabular}{@{}l|cc@{}}
\toprule
\textbf{Metric} & Accuracy & $\kappa$ \\
\midrule
Physics Accuracy & 67.3 & 0.231 \\
Prompt Adherence & 71.4 & 0.284 \\
Visual Realism & 91.8 & 0.000 \\
Motion Quality & 91.8 & 0.000 \\
\midrule
\textbf{Overall Score} & 91.8 & 0.000 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/prompt_index.tex <==
\begin{table*}[t!]
\centering
\caption{Index of all task prompts in the appendix. Each task includes video generation, image generation, and evaluation prompts detailed in their respective sections.}
\label{tab:prompt_index}
\small
\begin{tabular}{llllll}
\toprule
\textbf{Task Name} & \textbf{Domain} & \textbf{Metric} & \textbf{Video Prompt} & \textbf{Image Prompt} & \textbf{Eval Prompt} \\
\midrule
\multicolumn{6}{l}{\textit{\textbf{Abstract Reasoning}}} \\
Maze & Abstract & Finish Task & \autoref{sec:maze_video_prompt} & \autoref{sec:maze_image_prompt} & \autoref{sec:maze_eval} \\
Sudoku & Abstract & Valid Solution & \autoref{sec:sudoku_video_prompt} & \autoref{sec:sudoku_image_prompt} & \autoref{sec:sudoku_eval} \\
ARC-AGI & Abstract & Valid Solution & \autoref{sec:arc_video_prompt} & \autoref{sec:arc_image_prompt} & \autoref{sec:arc_eval} \\
Math & Abstract & Valid Solution & \autoref{sec:math_video_prompt} & \autoref{sec:math_image_prompt} & \autoref{sec:math_eval} \\
\midrule
\multicolumn{6}{l}{\textit{\textbf{Embodied Navigation}}} \\
Top-down View Navigation & Navigation & Reach Goal & \autoref{sec:topdown_video_prompt} & \autoref{sec:topdown_image_prompt} & \autoref{sec:topdown_eval} \\
3D Real-World Navigation & Navigation & Success & \autoref{sec:3dnav_video_prompt} & \autoref{sec:3dnav_image_prompt} & \autoref{sec:3dnav_eval} \\
Last-Mile Nav. (Ego-centric) & Navigation & Success & \autoref{sec:fpv_video_prompt} & \autoref{sec:fpv_image_prompt} & \autoref{sec:fpv_eval} \\
Simultaneous Localization and Generation & Navigation & Success & \autoref{sec:slag_video_prompt} & \autoref{sec:slag_image_prompt} & \autoref{sec:slag_eval} \\
\midrule
\multicolumn{6}{l}{\textit{\textbf{Physical Commonsense}}} \\
Physical Commonsense & Physics & Plausibility & \autoref{sec:physics_video_prompt} & \autoref{sec:physics_image_prompt} & \autoref{sec:physics_eval} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/sudoku_agreement_results.tex <==
\begin{table}[t]
\centering
\small
\caption{Human–evaluator agreement on the \textbf{Sudoku} task across three video models (n=253 total samples). We report raw agreement accuracy (\%) and Cohen's $\kappa$ for each evaluation metric.}
\vspace{-2mm}

\begin{subtable}{\columnwidth}
\centering
\caption*{(Top) Human vs. OCR-based Evaluator}
\vspace{-2mm}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
& \multicolumn{2}{c|}{\textbf{CC}} & \multicolumn{2}{c|}{\textbf{CV}} &
  \multicolumn{2}{c|}{\textbf{CA}} & \multicolumn{2}{c|}{\textbf{AR}} &
  \multicolumn{2}{c}{\textbf{OS}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & Acc. & $\kappa$ & Acc. & $\kappa$ & Acc. & $\kappa$
& Acc. & $\kappa$ & Acc. & $\kappa$ \\
\midrule
Sora-2  & 70.6 & 0.412 & 52.9 & 0.089 & 64.7 & 0.241 & 82.4 & 0.000 & 100.0 & 1.000 \\
Veo-3   & 65.1 & 0.302 & 48.8 & 0.042 & 58.1 & 0.178 & 79.1 & 0.000 & 100.0 & 1.000 \\
Wan-2.2 & 72.3 & 0.448 & 55.3 & 0.115 & 61.7 & 0.203 & 85.1 & 0.000 & 100.0 & 1.000 \\
\midrule
\textbf{Avg.} & 69.3 & 0.387 & 52.3 & 0.082 & 61.5 & 0.207 & 82.2 & 0.000 & 100.0 & 1.000 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{subtable}

\vspace{1mm}

\begin{subtable}{\columnwidth}
\centering
\caption*{(Bottom) Human vs. VLM-based Evaluator}
\vspace{-2mm}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
& \multicolumn{2}{c|}{\textbf{CC}} & \multicolumn{2}{c|}{\textbf{CV}} &
  \multicolumn{2}{c|}{\textbf{CA}} & \multicolumn{2}{c|}{\textbf{AR}} &
  \multicolumn{2}{c}{\textbf{OS}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & Acc. & $\kappa$ & Acc. & $\kappa$ & Acc. & $\kappa$
& Acc. & $\kappa$ & Acc. & $\kappa$ \\
\midrule
Sora-2  &  &  &  &  &  &  &  &  &  &  \\
Veo-3  &  &  &  &  &  &  &  &  &  &  \\
Wan-2.2 &  &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{Avg.} &  &  &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{subtable}
\vspace{-5mm}
\label{tab:sudoku_agreement_combined}
\end{table}

==> tables/sudoku_human_results.tex <==
\begin{table*}[h!]
\centering
\small
\caption{Comparison of \textbf{Auto-Eval} (VLM-based) and \textbf{Human-Eval} results for \textbf{Veo-3} on the Sudoku task across two grid sizes (4$\times$4, 9$\times$9) across three difficulty levels (Easy, Medium, and Hard).}
\label{tab:sudoku_human_results}
\begin{adjustbox}{max width=0.98\textwidth}
{
    \begin{tabular}{@{}llccccc@{}}
    \toprule
    & & \multicolumn{4}{c}{\textbf{Fine-grained Metrics}} & \multicolumn{1}{c}{\textbf{Primary Metric}} \\
    \cmidrule(lr){3-6} \cmidrule(lr){7-7}
    \textbf{Grid} & \textbf{Eval Type}
    & \textbf{Clues Changed} $\downarrow$
    & \textbf{Constraints Violation} $\downarrow$
    & \textbf{Completion Accuracy} $\uparrow$
    & \textbf{Action Reflection} $\uparrow$
    & \textbf{Overall} $\uparrow$ \\
    \midrule

    \multicolumn{7}{@{}l}{\textit{Level: Easy}} \\
    4$\times$4 & Auto-Eval
        & 27.60\% & 42.00\% & 37.21\% & 92.00\% & 11.38\% \\
               & Human-Eval
        & 86.67\% & 93.33\% & 0.00\% & 100.00\% & 0.00\% \\
    9$\times$9 & Auto-Eval
        & 31.60\% & 39.60\% & 15.47\% & 70.00\% & 3.18\% \\
               & Human-Eval
        & 60.00\% & 100.00\% & 0.00\% & 93.33\% & 0.00\% \\
    \midrule

    \multicolumn{7}{@{}l}{\textit{Level: Medium}} \\
    4$\times$4 & Auto-Eval
        & 24.40\% & 43.53\% & 37.61\% & 95.60\% & 9.70\% \\
               & Human-Eval
        & 100.00\% & 100.00\% & 0.00\% & 100.00\% & 0.00\% \\
    9$\times$9 & Auto-Eval
        & 34.00\% & 40.59\% & 13.66\% & 72.00\% & 2.77\% \\
               & Human-Eval
        & 66.67\% & 100.00\% & 0.00\% & 66.67\% & 0.00\% \\
    \midrule

    \multicolumn{7}{@{}l}{\textit{Level: Hard}} \\
    4$\times$4 & Auto-Eval
        & 30.12\% & 44.88\% & 30.50\% & 95.18\% & 8.71\% \\
               & Human-Eval
        & 40.00\% & 93.33\% & 0.00\% & 100.00\% & 0.00\% \\
    9$\times$9 & Auto-Eval
        & 31.20\% & 43.01\% & 13.45\% & 70.40\% & 2.57\% \\
               & Human-Eval
        & 53.33\% & 100.00\% & 0.00\% & 86.67\% & 0.00\% \\

    \bottomrule
    \end{tabular}
}
\end{adjustbox}
\end{table*}

==> tables/sudoku_statistics.tex <==
% \begin{table*}[h]
% \centering
% \small
% \caption{Sample distribution of the Sudoku task across difficulty levels and grid sizes. Each cell shows the number of puzzle instances. The total dataset comprises 300 Sudoku puzzles with balanced representation across both grid configurations and difficulty levels.}
% \label{tab:sudoku_distribution}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Difficulty Level} & \textbf{4×4 Grid} & \textbf{9×9 Grid} \\
% \midrule
% Easy & 50 & 50 \\
% Medium & 50 & 50 \\
% Hard & 50 & 50 \\
% \midrule
% \textbf{Total} & 150 & 150 \\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}
% \small
% \item \textbf{Note:} Difficulty levels are determined by the number of initial clues (pre-filled digits): \textit{Easy} puzzles provide dense clues, \textit{Hard} puzzles provide minimal clues while ensuring a unique solution. The 4×4 grids use digits 1–4 with 2$\times$2 subgrids; 9×9 grids use digits 1–9 with 3$\times$3 subgrids.
% \end{tablenotes}
% \end{table*}
